Extending the Range of Robust PCE Inflation Measures

Robust inflation measures gauge inflation behavior by excluding volatile expenditure categories from headline inflation. We evaluate the forecasting performance of a wide set of such measures between 1970 and 2024, including core, median, and trimmed mean personal-consumption-expenditure (PCE) inflation. Core inflation performs significantly worse than official median and trimmed mean inflation. Among a set of alternative trimmed mean measures, there is no single best trim based on forecasting performance: A wide set of trims generates statistically indistinguishable average errors. Nonetheless, different trims imply different predictions for trend inflation in any given month, within a range of 0.5 to 1 percentage points. In tracking trend inflation, this range and its midpoint outperform all trimmed mean inflation measures, suggesting the use of the range of inflation implied by the set of near-optimal trims as a valuable complement to any single inflation measure.

==> Tables/d31m_VOX.tex <==




\renewcommand{\tabcolsep}{15pt}
\begin{table}[tbh]
    \caption{Summary Statistics - Inflation Measures}
    \begin{center}
    \begin{threeparttable}
    \begin{tabular}{l cccc}
        \hline \hline
         & \multicolumn{4}{c}{Inflation Measures} \\
         & \multirow{2}{*}{Headline} & \multirow{2}{*}{Core} & \multirow{2}{*}{Median} & Trimmed \\
         &     &      &        & Mean    \\
        \cline{2-5}
         & \multicolumn{4}{c}{Full Sample (748 months)}\\
        \cline{2-5}
        Mean        & 3.27  &  3.21  &  3.33  &  2.96 \\
        Std. Dev.   & 2.42  &  2.13  &  2.01  &  1.86 \\
        Coeff. Var. & 0.74  &  0.66  &  0.60  &  0.63 \\
        \cline{2-5}
         & \multicolumn{4}{c}{low inflation: $\pi<2.5\%$ (373 months)}\\
        \cline{2-5}
        Mean        & 1.55  &  1.73  &  2.01  &  1.72 \\
        Std. Dev.   & 0.67  &  0.53  &  0.95  &  0.70 \\
        Coeff. Var. & 0.43  &  0.31  &  0.47  &  0.41 \\
        \cline{2-5}
         & \multicolumn{4}{c}{medium inflation: $2.5\%\leq\pi<5\%$ (252 months)}\\
        \cline{2-5}
        Mean        & 3.61  &  3.51  &  3.55  &  3.17 \\
        Std. Dev.   & 0.71  &  1.06  &  0.84  &  0.77 \\
        Coeff. Var. & 0.20  &  0.30  &  0.24  &  0.24 \\
        \cline{2-5}
         & \multicolumn{4}{c}{high inflation: $5\%\leq\pi$ (123 months)}\\
        \cline{2-5}
        Mean        & 7.76  &  7.09  &  6.85  &  6.31 \\
        Std. Dev.   & 2.00  &  1.59  &  1.60  &  1.57 \\
        Coeff. Var. & 0.26  &  0.22  &  0.23  &  0.25 \\
        \hline
    \end{tabular}
    \begin{tablenotes}
        \item {\footnotesize \textit{Notes:} The numbers are mean, standard deviation, and coefficient of variation of the different inflation measures for different samples determined by the level of PCE inflation. All numbers are in percentage points.}
    \end{tablenotes}
    \end{threeparttable}
    \end{center}
    \label{tab:Mean_StD_Inflation}
\end{table} 
\renewcommand{\tabcolsep}{10pt}




